Derivative-Free Global Minimization in One Dimension: Relaxation, Monte Carlo, and Sampling

We introduce a derivative-free global optimization algorithm that efficiently computes minima for various classes of one-dimensional functions, including non-convex, and non-smooth functions.This algorithm numerically approximates the gradient flow of a relaxed functional, integrating strategies such as Monte Carlos methods, rejection sampling, and adaptive techniques. These strategies enhance performance in solving a diverse range of optimization problems while significantly reducing the number of required function evaluations compared to established methods. We present a proof of the convergence of the algorithm and illustrate its performance by comprehensive benchmarking. The proposed algorithm offers a substantial potential for real-world models. It is particularly advantageous in situations requiring computationally intensive objective function evaluations.

==> tables/restart <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}\hline\(options\)&\(n_f\)&\(\Pi\)&\(\Pi_{100}\)&\(\tau\)&\(n\)&\(\Delta\)&\(\Delta_c\)\\\hline\(<||>\)&\(148.7\)&\(0.93\)&\(0.84\)&\(0.3\)&\(205.4\)&\(0.015\)&\(0.000016\)\\\hline\(<|restart -> False|>\)&\(105.6\)&\(0.82\)&\(0.81\)&\(0.27\)&\(145.\)&\(0.027\)&\(0.000036\)\\\hline\end{tabular}

==> tables/restartedited.tex <==
\begin{tabular}{|c|c|c|c|c|c|c|c|}\hline Restart &\(n_f\)&\(\Pi\)&\(\Pi_{100}\)&\(\tau\)&\(n\)&\(\Delta\)&\(\Delta_c\)\\\hline 
True&\(207.1\)&\(0.93\)&\(0.72\)&\(0.34\)&\(186.1\)&\(0.016\)&\(0.00002\)\\\hline
%True &\(208.2\)&\(0.93\)&\(0.72\)&\(0.29\)&\(180.\)&\(0.016\)&\(0.000023\)\\\hline
False &\(133.3\)&\(0.83\)&\(0.73\)&\(0.16\)&\(107.4\)&\(0.028\)&\(0.000041\)\\\hline\end{tabular}
